Rapid prediction of lab-grown tissue properties using deep learning

The interactions between cells and the extracellular matrix are vital for the self-organisation of tissues. In this paper we present proof-of-concept to use machine learning tools to predict the role of this mechanobiology in the self-organisation of cell-laden hydrogels grown in tethered moulds. We develop a process for the automated generation of mould designs with and without key symmetries. We create a large training set with $N=6500$ cases by running detailed biophysical simulations of cell-matrix interactions using the contractile network dipole orientation (CONDOR) model for the self-organisation of cellular hydrogels within these moulds. These are used to train an implementation of the \texttt{pix2pix} deep learning model, reserving $740$ cases that were unseen in the training of the neural network for training and validation. Comparison between the predictions of the machine learning technique and the reserved predictions from the biophysical algorithm show that the machine learning algorithm makes excellent predictions. The machine learning algorithm is significantly faster than the biophysical method, opening the possibility of very high throughput rational design of moulds for pharmaceutical testing, regenerative medicine and fundamental studies of biology. Future extensions for scaffolds and 3D bioprinting will open additional applications.

==> extratext_placeholder.tex <==
[TEXT FROM ]

Continuum models have been developed to describe the alignment of stress fibers in artificial tissue constructs through both passive elasticity and the active forces generated by cells \cite{deshpande2006,pathak2008,obbinkhuizer2014}. Legand {\it et al.} \cite{legand2009} have compared the continuum model of Refs. \cite{deshpande2006,pathak2008} with artificial tissue structures grown in MEMS systems, finding good agreement between model and experiment.  Continuum models necessarily coarse grain cells and ECM into a single effective material containing the properties of both cells and ECM. Once this has been done, cells cannot be individually tracked, and cell alignments are assumed to follow stress fibers directly. A description of tissues as active continuum materials is well suited for modeling situations where the properties of individual cells are not important.

Microscopic models are complementary, but distinct to, continuum approaches. In a microscopic model, it is possible to model the complex self-organization of an ensemble of distinct cells in response to their environments, without the coarse graining associated with continuum models, and thus allowing simulations to be carried out that treat processes on cellular length scales. On the other hand, a typical challenge for microscopic models is carrying out simulations that are large enough to capture macroscopic scales.

{\fp To develop a microscopic model of ECM-cell interactions leading to self-organization, that can be simulated on macroscopic scales, we take inspiration from force-dipole models and contractile network models.} A force-dipole approach could be used to simulate the interactions between cells and the ECM (see e.g. \cite{schwarz2013}). Since it has been established that cells find an orientation consistent with the minimum work needed to obtain that configuration \cite{bischofs2003}, it would then suffice to find the lowest energy (ground) state of the theoretical model. However, the cells in such force-dipole models must be constrained to occupy nearly-fixed positions in their substrates to avoid volume collapse relating to the form of the interaction (which has a $1/r^3$ attractive form). Thus, such models cannot describe the reshaping of tissue that occurs simultaneously with self-organization. We also take inspiration from contractile network models, in which networks of springs can be used to model elastic effects in e.g. biopolymers \cite{guthardttorres2012,boal}. To date, the active forces due to cell-ECM interaction have not been introduced into contractile network models.


{\fp Our COntractile Network Dipole ORentiation (CONDOR) model of cellular self-organization goes beyond previous work by combining force-dipole orientation models with contractile network models.}  Our microscopic model combines a complex network of elastic fibers that represents the ECM, with active forces that follow cell symmetries, to describe the active feedback between cells and ECM. This active feedback leads and responds to the macroscopic self-organization and reshaping of tissues. It is able to describe the tension fields, self-organization, and reshaping of tissues that arise from the active forces between cells and ECM.  Spring networks are a popular way of representing elasticity in biopolymers \cite{boal}, and force-dipoles are a successful way of representing ordering of cells in tissues \cite{schwarz2013}, but the two approaches have not yet been combined in this way. 


{\fp Beyond the biophysical description of complexity in tissues, our CONDOR model could assist in the rational design of the scaffolds and molds that direct self-organization in engineered (or artificial) tissues.} Artificial tissues are important in both pharmaceutical testing and regenerative medicine. In order to be useful for these applications, engineered tissues need to mimic the properties of real tissues. For example, it is critical that cells in artificial nervous and corneal tissues are  self-organized so that they are highly aligned \cite{georgiou2013,phillips2005,mukhey2018,east2010}. 
The development of new molds and scaffolds to encourage biologically relevant self-organization can take many months or years of painstaking trial and error. Thus, there is a need for new biophysical models capable of simulating the onset of self-organization in artificial tissues, which can be used for predicting which mold and scaffold designs have a good chance of success. Hence, our secondary goal is to generate techniques for detailed large-scale simulations of self-organization in artificial tissues that can be used as tools to assist rational design of molds and scaffolds.

{\fp Our CONDOR model has several key strengths, including:}
\begin{enumerate}
\item Accurate description of the self-organization and reshaping of tissue that is driven by the feedback between cells and ECM.

\item Predictive capability for the shapes of tissues and the orientations of cells in those tissues.

\item Simplicity allows for simulation of large numbers of cells allowing macroscopic tissue sizes to be approached.

\item Generalizability to different symmetry arrangements by adding higher order multipolar corrections or other alternative symmetries to $f(\theta)$ to allow the investigation of other biophysics.

\item Extensibility to disorder, which can be achieved by including random bonds or
by making corrections to the equilibrium distances of bonds. 

\item  Similarities to models common in statistical phsyics (such as the Heisenberg model of spin alignments, and models of liquid crystals), allowing the extensive machinery of statistical physics to be used to solve the microscopic model (e.g. Monte Carlo methods).
\end{enumerate}

\subsection{Potential applications of the model}

{\fp Specific patterns of cellular self-organization are important in many tissues, making it challenging to grow artificial tissues that properly represent those in living organisms. } The use of artificial or engineered tissue for regenerative medicine has the potential to significantly improve human health \cite{obrien2011} and provide new biological models for drug testing \cite{orourke2017}. The cells in real tissues are typically arranged in ways that may be difficult to reproduce artificially. For example, this is a particular problem for nerve tissue, which must be well-ordered to function properly. In the nervous system, neurons are typically guided by glial cells, so well-ordered glial cells in artificial tissue could lead to well-directed neuron growth for, e.g., nerve repair. For such applications, favorable characteristics are high levels of cell alignment and cross-section that is uniform along the length of the  tissue, while regions of misalignment around tethering points should be minimized. 


{\fp  Design of artificial tissue with realistic characteristics is something that is very difficult and time consuming to do experimentally using trial and error, so the ability to predict outcomes would be extremely valuable.} 
The CONDOR model described here is fast enough to  assist the rational design of experimental molds and scaffolds that guide artificial tissue growth. The comparison with experiment carried out here indicates that for a design process, a broad range of $\Delta$ should be used to obtain indicative results for specific mold designs.

\subsection{Future prospects}

{\fp  Future work will increase sophistication of the CONDOR model to improve predictions of self-organization in tissue.} There are several ways in which the model could be extended:

1. Improved cell response to tension in the ECM: The cells in the CONDOR model are always elongated (polarized), however experimental systems have regions where cells are not elongated, particularly within the Delta region, so the contraction of the sample may be over-estimated. The CONDOR model could be modified so cells are unpolarized in regions of low tension.

2. Increased sophistication to improve the description of the ECM and analyse the role of disorder: For example, the polymers making up the ECM have many signatures of disorder.  Randomized spring networks could therefore improve the description of collagen networks in the ECM. An intriguing possibility for further physics investigation, is the existence of phase transitions between self-organization and disorder in the CONDOR model. 

3. Inclusion of time dependence: Cell representations in the model could be extended to include dynamic responses. This would allow the study of time-dependent ECM remodeling, the evolution of samples during their growth phase \cite{orourke2015}, or oscillatory strain stimuli (e.g. \cite{de2007,de2008,safran2009}).
 
Our microscopic model is amenable to all of these extensions and work is currently in progress. Overall, we expect that a wide range of interesting biophysics can be studied within extensions to the CONDOR model introduced here.

